Measuring Non-Expert Comprehension of Machine Learning Fairness Metrics

Bias in machine learning has manifested injustice in several areas, such as medicine, hiring, and criminal justice. In response, computer scientists have developed myriad definitions of fairness to correct this bias in fielded algorithms. While some definitions are based on established legal and ethical norms, others are largely mathematical. It is unclear whether the general public agrees with these fairness definitions, and perhaps more importantly, whether they understand these definitions. We take initial steps toward bridging this gap between ML researchers and the public, by addressing the question: does a lay audience understand a basic definition of ML fairness? We develop a metric to measure comprehension of three such definitions--demographic parity, equal opportunity, and equalized odds. We evaluate this metric using an online survey, and investigate the relationship between comprehension and sentiment, demographics, and the definition itself.

==> Describing Fairness ICML20 (1)_arXiv/acknowledgments.tex <==
\section*{Acknowledgments}
\jpd{Apparently these don't count toward the page limit for the body of the paper, ``It has now been decided that the acknowledgments section might appear after the 9th page (along with references). The paper checker has been updated accordingly.''}
Dickerson, McElfresh, and Schumann were supported in part by NSF CAREER Award IIS-1846237, DARPA GARD Award \#HR112020007, DARPA SI3-CMD Award \#S4761, DoD WHS Award \#HQ003420F0035, NIH R01 Award NLM-013039-01, and a Google Faculty Research Award.
We gratefully acknowledge funding support from the NSF (Grants 1844462 and 1844518).
The opinions in this paper are those of the authors and do not necessarily reflect the opinions of any funding sponsor or the United States Government.


==> Describing Fairness ICML20 (1)_arXiv/demo.tex <==
Table~\ref{tab:demo} summarizes the ethnicity and education level of participants in both \studyA{} and \studyB{}.

\begin{table}[ht]
\centering
\caption{\label{tab:demo} Participant demographics across ethnicity and education level, compared to the 2017 U.S. Census. AI = American Indian, AN = Alaska Native, NH = Native Hawaiian, PI = Pacific Islander, AA = African American. Note that in \studyB{}, two participants did not report their education level.}
\vspace{5pt}
{\small
\begin{tabular}{@{}lrrr@{}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Percent of Sample}} \\
    & \textbf{Census} & \textbf{\studyA{}} & \textbf{\studyB{}} \\
    \midrule
    \textbf{Ethnicity} & & \\
    AI or AN & 0.7 & 0.7 & 0.9\\
    Asian or NH or PI & 5.7 & 1.4 & 2.3 \\
    Black or AA & 12.3 & 10.2 & 15.8 \\
    Hispanic or Latinx & 18.1 & 12.2 & 7.7\\
    Other & 2.6 & 2.7 & 1.4 \\
    White & 60.6 & 72.8 & 71.9 \\
    
  \addlinespace[1.5 ex]
    \textbf{Education Level} & & \\
    Less than HS & 12.1 & 6.1 & 6.9 \\
    HS or equivalent & 27.7 & 29.9 & 24.9 \\
    Some post-secondary & 30.8 & 30.6 & 24.9 \\
    Bachelor's and above & 29.4 & 33.3 & 42.7 \\
    \bottomrule
\end{tabular}%
}
\vspace{-5pt}
\end{table}

==> Describing Fairness ICML20 (1)_arXiv/studyA_results.tex <==
\subsection{Our Survey Effectively Captures Rule Comprehension} \label{results:1:rq1}

We find that our survey is internally consistent, and effectively measures participant comprehension of demographic parity. The former we evaluated using Cronbach's $\alpha$ and item-total correlation (discussed in \S\ref{results:a:validity}), and the latter using two self-report measures and one free response question.
See Fig.~\ref{fig:question_breakdown} for participant performance per question.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/question_breakdown.png}
    \vspace{-10pt}
    \caption{Number of participants answering each question correctly. Each panel contains all 147 participants. 
    }
    \label{fig:question_breakdown}
    \vspace{-5pt}
\end{figure}


\subsubsection{Self-reported rule understanding and use are reflected in comprehension score}
First, we compared comprehension score to self-reported rule understanding (Q13). Higher comprehension scores were associated with greater confidence in understanding (Spearman's rho), suggesting that participants were accurately assessing their ability to apply the rule (see Fig. \ref{fig:q13}).





\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/q13.png}
    \vspace{-10pt}
    \caption{Comprehension score grouped by response to Q13. Self-reported understanding of the rule was associated with higher comprehension scores. X-axis is reversed for figure and correlation test.}
    \label{fig:q13}
\end{figure}



Next, we compared comprehension score to a self-report question about the participant's use of the rule (Q14)
Participants who claimed to use only the rule tended to score higher than those who used their own notions of fairness or a combination thereof (K-W test, and post-hoc M-WU), suggesting that participants are answering somewhat honestly: when they try to apply the rule, comprehension scores improve (see Fig.~\ref{fig:q14}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/q14.png}
    \vspace{-10pt}
    \caption{Comprehension score grouped by response to Q14. Rule compliance (leftmost on the x-axis) was associated with higher comprehension scores. One participant who did not provide a response was excluded from the figure and relevant analysis.}
    \label{fig:q14}
\end{figure}



\subsubsection{Participants with higher comprehension scores are better able to explain the rule}
To further validate our comprehension score, we asked participants to explain the rule in their own words (Q12). %
Responses were qualitatively coded as one of five categories: \textbf{correct}, \textbf{partially correct}, \textbf{neither}, \textbf{incorrect}, or \textbf{none} (as discussed in \S\ref{results:a:validity}). The results of this coding can be seen can be seen in Fig. \ref{fig:q12}. Participants providing correct explanations of the rule attained higher comprehension scores (k-W test, and post-hoc M-WU), further corroborating our claim that our comprehension score is a valid measure of fairness rule comprehension.


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/q12.png}
    \vspace{-10pt}
    \caption{Comprehension score grouped by code assigned to Q12 response. Participants who provided either correct or partially correct responses tended to perform better.}
    \label{fig:q12}
    \vspace{-10pt}
\end{figure}



\subsection{Education Influences Comprehension} \label{results:1:rq2}

During the cognitive interview phase, we observed a possible trend of comprehension scores being lower for older participants and those with less educational attainment. If true, this would suggest that fairness explanations should be carefully validated to ensure they can be used with diverse populations. We investigated this hypothesis, in an exploratory fashion, using poisson regression models.

Three models were tested. The first regressed score against all four demographic categories as predictors (gender, age, ethnicity, and education), the second omitted education, and the third tested only education. Models were compared using Akaike information criterion (AIC), a standard method of evaluating model quality and performing model selection \cite{akaike1974}. Comparison by AIC revealed that model 1 (all four categories) was a better predictor for comprehension score than models 2 or 3 (AIC = 643.3, 651.2, and 660.5, respectively; difference = 0.0, 7.9, and 17.1). 
In model 1, only education showed correlation with comprehension score (effect size = $1.40$, $p<0.05$). %
Further work is needed to confirm this exploratory result.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/edu.png}
    \vspace{-10pt}
    \caption{Comprehension score grouped by education level. Higher education level was associated with higher comprehension scores.}
    \label{fig:edu}
    \vspace{-10pt}
\end{figure}

\subsection{Disagreement with the Rule is Associated with Higher Comprehension Scores} \label{results:1:rq3}

Participants were asked for their opinion on the presented rule in another free response question (Q15). These responses were then qualitatively coded to capture participant sentiment towards the rule as one of five categories: \textbf{agree}, \textbf{depends}, \textbf{disagree}, \textbf{not understood}, or \textbf{none} (as discussed in \S\ref{results:a:hypotheses}).

 
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/q15.png}
    \caption{Comprehension score grouped by code assigned to Q15 response. Participants who exhibited negative sentiment toward the rule responses tended to perform better.}
    \label{fig:q15}
    \vspace{-10pt}
\end{figure}
This question was added based on the cognitive interviews (see \Appref{methods:design:cog}), where perception seemed to influence compliance.
The results of coding Q15 can be seen in Fig. \ref{fig:q15}. Participants who expressed disagreement with the rule performed better than those who expressed agreement, did not understand the rule, or provided no response to the question (K-W test, post-hoc M-WU). Note that this result should not be interpreted as an overall finding on the appropriateness of demographic parity. Instead we anticipate the perceptions of appropriateness of any fairness definition will be highly context-dependent.





\subsection{Non-Compliance is Associated with Lack of Understanding} \label{results:a:non-comp}

We were interested in understanding why some participants failed to adhere to the rule, as measured by their self-report of rule usage in Q14. 
After labeling participants as either ``non-compliant" (NC, $n=57)$ or ``compliant" (C, $n=89$), we conducted a series of $\chi^2$ tests to investigate this phenomenon.

Non-compliant participants were less likely to self-report high understanding of the rule in Q13 (see Fig. \ref{fig:q13q14}). %
Moreover, non-compliance also appears to be associated with a reduced ability to correctly explain the rule in Q12 (see Fig. \ref{fig:q12q14}). %
Further, negative participant sentiment towards the rule (Q15) also appears to be associated with greater compliance (see Fig. \ref{fig:q15q14}). %
Thus, non-compliant participants appear to behave this way because they do not \emph{understand} the rule, rather than because they do not \emph{like} it. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/nc_q13q14.png}
    \vspace{-15pt}
    \caption{Self-report of understanding (Q13) split by compliance (Q14). NC participants tend to report less confidence in their ability to apply the rule. SD = strongly disagree, D = disagree, N = neither agree nor disagree, A = agree, SA = strongly agree.}
    \label{fig:q13q14}
    \vspace{-5pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/nc_q12q14.png}
    \vspace{-15pt}
    \caption{Correctness of rule explanation (Q12) split by compliance (Q14). NC participants tend to be less able to explain the presented rule in their own words. NA = none, I = incorrect, N = neither, PC = partially correct, C = correct.}
    \label{fig:q12q14}
    \vspace{-5pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/nc_q15q14.png}
    \vspace{-15pt}
    \caption{Participant agreement with rule (Q15) split by compliance (Q14). NC participants tend to harbor less negative sentiment towards the rule. NA = none, NU = not understood, D = disagree, De = depends, A = agree.}
    \label{fig:q15q14}
    \vspace{-5pt}
\end{figure}



==> Describing Fairness ICML20 (1)_arXiv/studyA_scenario_analysis.tex <==

\subsection{Decision Scenarios} \label{app:scenario_analysis}

For \studyA{} we designed three decision-making scenarios to test whether the perceived importance or realism of a particular scenario influenced comprehension score. They are as follows:
\begin{itemize} \itemsep=0cm
    \item \textbf{Art Project (AP):} distributing awards for art projects to primary school students,
    \item \textbf{Employee Awards (EA):} distributing employee awards at a sales company, and
    \item \textbf{Hiring (HR):} distributing job offers to applicants.
\end{itemize}
In each scenario the students/employees/applicants are partitioned into two groups (parents' occupation for the first scenario, and binary gender for the other two scenarios).
We use a between-subjects design: participants are randomly partitioned into three conditions, one for each scenario (AP, EA, or HR).
For each condition we define the \emph{fairness rule} in the context of the decision-making scenario (see Appendix~\ref{app:survey} for the full surveys).

Next we describe our main conclusion related to the different decision-making scenarios in \studyA: the scenario does not influence comprehension score.


\subsubsection{Scenario does not Influence Comprehension Scores (RQ4)} \label{results:rq4}

We were concerned that less important and/or realistic scenarios would cause participants to take the survey less seriously, and therefore perform more poorly.
To test this,
participants were randomly assigned to a scenario, resulting in the following distribution: AP = 41, EA = 49, HR = 57.

A K-W test revealed no differences between scenarios in terms of comprehension score (mean comprehension scores: AP = 6.0, EA = 6.74, HR = 5.86%
). However, differences did exist between scenarios in terms of importance (assessed in Q2), measured in hours of effort deemed necessary to make the relevant decision (K-W, %
$p<0.001$). Post-hoc M-WU revealed that participants believed making a decision in the AP scenario merited fewer hours of effort (mean = 3.15hrs) than in the EA (13.52hrs, $p<0.001$)
or HR (15.23hrs, $p<0.001$)
scenarios (corrected $\alpha=0.05/3=0.017$). See Fig. \ref{fig:q2} for distributions of responses.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/q2.png}
    \vspace{-10pt}
    \caption{Importance of a scenario by proxy of hours of effort necessary to make a decision in each scenario. AP merited less hours of effort than both EA and HR.}
    \label{fig:q2}
\end{figure}

Of note, it is possible that perceived realism, assessed in Q1 on a five-point Likert scale, was also influenced by scenario (K-W, $p=0.051$), but we may need larger sample sizes to confirm this. Regardless, while the nature of a scenario does influence participant perception in terms of importance and (possibly) realism, it does not appear to influence comprehension (at least for the scenarios we chose). For this reason, we chose to test a single scenario (HR) in \studyB{}. %


==> Describing Fairness ICML20 (1)_arXiv/studyB_details.tex <==
\subsection{Model Selection} \label{app:b:model_selection}

In \S\ref{results:b:edu} we assessed eleven linear regression models for predicting comprehension scores. The best fit model, determined by model selection via AIC, included only education (edu) and fairness definition (def) as regressors. The results of model selection are below in Table \ref{tab:AIC}.

\begin{table}[bht]
\centering
\caption{\label{tab:AIC} Models tested in \S\ref{results:b:edu}, sorted by best to least fit. The first model in the table (edu + def) is the model of best fit. dAIC = difference from model with lowest AIC value.}
\vspace{7pt}
{\small
\begin{tabular}{@{}lrr@{}}
    \toprule
    \textbf{Model regressors} & \textbf{AIC} & \textbf{dAIC} \\
    \midrule
    edu + def & -80.4 & 0 \\
    edu & -72.8 & 7.6 \\
    gender + edu & -70.3 & 10.1 \\
    age + edu & -63.7 & 16.7 \\
    gender + age + edu & -61.1 & 19.2 \\
    gender + age + eth + edu + def & -61.1 & 19.2 \\
    def & -60.8 & 19.6 \\
    gender + age + eth + edu & -55.5 & 24.9 \\
    gender + age + def & -46.4 & 34 \\
    gender + age + eth + def & -41.6 & 38.8 \\
    gender + age + eth & -37.2 & 43.2 \\
    \bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table}

\subsection{Non-Compliance} \label{app:b:compliance}

In \S\ref{results:b:non-comp} we sought to further investigate the findings of \studyA{} with regards to compliance (Q14). To do so, we labeled those who responded (in \studyB{}) with either having used their own personal notions of fairness ($n=26)$ or some combination of their personal notions and the rule ($n=148$) as ``non-compliant" (NC), with the remaining $n=174$ labeled as ``compliant" (C). One participant who did not provide a response was excluded from this analysis, conducted using KW and $\chi^2$ tests.

Non-compliant participants were less likely to self-report high understanding of the rule in Q13 %
(KW test, $p<0.001$, see Fig. \ref{fig:studyB_nc_q13q14}). Moreover, non-compliance also appears to be associated with a reduced ability to correctly explain the rule in Q12 %
($\chi^2$ test, $p<0.001$, see Fig. \ref{fig:studyB_nc_q12q14}). This fits with the overall strong relationship we observed among comprehension scores, %
ability to explain the rule, and compliance. 

Further, greater dislike towards the rule (Q15) also appears to be associated with greater compliance %
(KW test, $p<0.05$, see Fig. \ref{fig:studyB_nc_q15q14}). %
However, there was no relationship between disagreement towards the rule (Q16) and compliance (see Fig. \ref{fig:studyB_nc_q16q14}).

These results largely corroborate the notion that non-compliant participants appear to behave this way because they do not \emph{understand} the rule, rather than because they do not \emph{like} it. %

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig_studyB/nc_q13q14.png}
    \vspace{-15pt}
    \caption{Self-report of understanding (Q13) split by compliance (Q14). NC participants tend to report less confidence in their ability to apply the rule. SD = strongly disagree, D = disagree, N = neither agree nor disagree, A = agree, SA = strongly agree.}
    \label{fig:studyB_nc_q13q14}
    \vspace{-5pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig_studyB/nc_q12q14.png}
    \vspace{-15pt}
    \caption{Correctness of rule explanation (Q12) split by compliance (Q14). NC participants tend to be less able to explain the presented rule in their own words. NA = none, I = incorrect, N = neither, PC = partially correct, C = correct.}
    \label{fig:studyB_nc_q12q14}
    \vspace{-5pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig_studyB/nc_q15q14.png}
    \vspace{-15pt}
    \caption{Participant liking for rule (Q15) split by compliance (Q14). NC participants tend to dislike the rule less than C participants. SD = strongly disagree, D = disagree, N = neither agree nor disagree, A = agree, SA = strongly agree.}
    \label{fig:studyB_nc_q15q14}
    \vspace{-5pt}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig_studyB/nc_q16q14.png}
    \vspace{-15pt}
    \caption{Participant agreement with rule (Q16) split by compliance (Q14). No differences were found between NC and C participants. SD = strongly disagree, D = disagree, N = neither agree nor disagree, A = agree, SA = strongly agree.}
    \label{fig:studyB_nc_q16q14}
    \vspace{-5pt}
\end{figure}

==> Describing Fairness ICML20 (1)_arXiv/studyB_survey.tex <==
Each of the surveys are split into four main sections. The first section is the consent form which can be found in Appendix~\ref{app:consent}. The second section describes the hiring scenario and asks questions about it (\S\ref{app:st2_scenarios}). The third section describes the fairness metric, defined as the rule, used (in this case it is demographic parity) and asks specific questions about the metric (\S\ref{app:st2_fairness}). Finally the last section asks for demographic information (\S\ref{app:demographics}).

\subsubsection{Scenario description and questions}\label{app:st2_scenarios}
The following is shown to each participant (note that Step 3 is not shown to participants with the DP definition):

It is very important that you read each question carefully and think about your answers. The success of our research relies on our respondents being thoughtful and taking this task seriously.
\begin{itemize}
    \vspace{-8pt}
    \item[\checkbox] I have read the above instructions carefully.
    \vspace{-8pt}
\end{itemize}

A company, Sales-a-lot, is reviewing their hiring process. They want to hire applicants who are high performing, and they also want to make sure that their hiring process is fair to their applicants, no matter their gender. To do this, Sales-a-lot employs an external firm, Recruit-a-matic, which keeps track of all applicants. This review will take place over one year.
 
For clarity at each stage of the hiring process we use images to represent the hiring pool.

\paragraph{Step 1: Applicant Pool.} At the beginning of the year, Sales-a-lot reviews all job applicants, and sends job offers to some of them. The initial applicant pool is shown with a gray background. For example, the following image shows an applicant pool with 15 female applicants and 25 male applicants:

\includegraphics[height=1in]{illustrations/intro/step_1_green_yellow.png}

\paragraph{Step 2: Sending Job Offers.} Next, Sales-a-lot sends job offers \space to some of these \space applicants, using the \space following criteria:
\begin{itemize} \itemsep=0pt
    \vspace{-10pt}
    \item Interview scores
    \item Quality of recommendation letters
    \item Number of years of prior experience in the field
\end{itemize}
Suppose that Sales-a-lot sends offers to 5 female applicants and 8 male applicants (so 10 female and 17 male applicants didn’t receive offers). In the following image, applicants who received a job offer are shown on the left (with a green background) and applicants who didn’t receive a job offer are shown on the right, with a red background):

\includegraphics[height=1in]{illustrations/intro/step_2_green_yellow_OFFER.png}
\space\space\space
\includegraphics[height=1in]{illustrations/intro/step_2_green_yellow_NO_OFFER.png}

\paragraph{Step 3: Applicant Evaluation.} For the rest of the year, Recruit-a-matic (the external firm) keeps track of all applicants in the initial pool, whether they received job offers or not. At the end of the year, Rectruit-a-matic finds out which applicants were high performers, i.e. qualified (shown in dark), and which applicants were low performers, i.e. unqualified (shown in light). For example, the following image shows that most of the high performers received job offers, but some did not.

\includegraphics[height=1in]{illustrations/intro/step_3_OFFER.png}
\space\space\space
\includegraphics[height=1in]{illustrations/intro/step_3_NO_OFFER.png}

\begin{tabular}{r|c|c}
     & female & male  \\
    \midrule
    qualified & \includegraphics[height=0.2in]{illustrations/intro/qual_female.png} & \includegraphics[height=0.2in]{illustrations/intro/qual_male.png} \\
    unqualified & \includegraphics[height=0.2in]{illustrations/intro/uqual_female.png} & \includegraphics[height=0.2in]{illustrations/intro/uqual_male.png} \\
\end{tabular}


\paragraph{Questions}
\begin{enumerate}
    \vspace{-5pt}
    \item To what extent do you agree with the following statement: a scenario similar to the one described above might occur in real life.
    \begin{itemize}
        \item Strongly agree
        \item Agree
        \item Neither agree nor disagree
        \item Disagree
        \item Strongly disagree
    \end{itemize}

    \item How much effort, in hours, should Sales-a-lot put in to make sure these decisions were fair? [short answer - number of hours]
\end{enumerate}

\subsubsection{Rule descriptions and questions}\label{app:st2_fairness}
The following sections provide fairness definitions (presented to participants as \emph{rules}) for Demographic Parity, Equal Opportunity (FNR and FPR), and Equalized Odds. Unless otherwise noted the rule description is shown above each of the questions for reference. Correct answers are noted in \correct{red}.

\paragraph{Demographic Parity.}

Recruit-a-matic uses the following rule to determine whether Sales-a-lot’s hiring decisions were fair:
 
\emph{The fraction of male candidates who receive job offers should equal the fraction of female candidates who receive job offers.}

Example 1: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot received the following applicants (10 female and 12 male).

\includegraphics[height=1in]{illustrations/demo_parity/example_1_POOL.png}

If Sales-a-lot sent job offers to the following number of applicants (5 female and 6 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/demo_parity/example_1b_offer.png}

Example 2: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot reviewed a total of 100 applicants as follows (40 female and 60 male).

\includegraphics[height=2in]{illustrations/demo_parity/example_2_POOL.png}

If Sales-a-lot sent job offers to the following number of applicants (10 female and 15 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/demo_parity/example_2b_offer.png}

In the next section, we will ask you some questions about the information you have just read. Please note that this is not a test of your abilities. We want to measure the quality of the description you read, not your ability to take tests or answer questions.

\textbf{Please note that we ask you to apply and use ONLY the above hiring rule when answering the following questions. You will have an opportunity to state your opinions and feelings on the rule later in the survey.}

\begin{enumerate}
\setcounter{enumi}{2}
    \item Suppose a different company considered applicants for a different job. There were 200 female applicants and 100 male applicants,

\includegraphics[height=1.3in]{illustrations/demo_parity/q3_POOL.png}

and they did send job offers to 90 male applicants.

\includegraphics[height=1.3in]{illustrations/demo_parity/q3_male_offer.png}

Assuming that Recruit-a-matic reviews their decisions using the hiring rule above, how many female applicants should have received job offers?
\begin{enumerate}
    \item 190
    \includegraphics[height=1.3in]{illustrations/demo_parity/q3_a_offer.png}
    \item \correct{180}
    \includegraphics[height=1.3in]{illustrations/demo_parity/q3_b_offer.png}
    \item 160
    \includegraphics[height=1.3in]{illustrations/demo_parity/q3_c_offer.png}
    \item 150
    \includegraphics[height=1.3in]{illustrations/demo_parity/q3_d_offer.png}
\end{enumerate}

\item Assuming Recruit-a-matic reviews decisions using the hiring rule above, in which of these cases could Sales-a-lot have accepted more qualified female applicants than qualified male applicants?

\begin{enumerate}
    \item When there are more qualified female applicants than qualified male applicants (i.e., more women had low net sales at the end of the year).
    \item \correct{When there are more female applicants than male applicants.}
    \item When female applicants receive worse interview scores than male applicants.
    \item This cannot happen under the hiring rule.
\end{enumerate}

\item Consider one male applicant and one female applicant, both of whom are similarly qualified for the job (they achieve about the same net sales at the end of their first year). Is the following statement \correct{TRUE} OR FALSE: The hiring rule above allows Sales-a-lot to make a job offer to one of these applicants and not the other.

\item Consider a situation where all female applicants were unqualified (they all achieve low net sales at the end of their first year), but some of them received job offers. Is the following statement TRUE OR \correct{FALSE}: The hiring rule above requires that some job offers made to male applicants must have been made to unqualified male applicants.

\item Suppose Sales-a-lot received 100 male and 100 female applicants, and eventually made 10 job offers. Is the following statement \correct{TRUE} OR FALSE: The hiring rule above requires that even if all male applicants were unqualified (they all achieve low net sales at the end of their first year), some of the unqualified males must have received job offers.

\item Is the following statement TRUE OR \correct{FALSE}: The hiring rule above always allows Sales-a-lot to send job offers only to the most qualified applicants (those who achieve high net sales at the end of their first year).

\end{enumerate}

Consider a different scenario than the two examples above, with 6 applicants -- 4 female and 2 male, as illustrated below. The next three questions each give a different potential outcome for all 6 applicants (i.e., which of the 6 applicants do receive job offers). Please indicate which of the outcomes follow the hiring rule above.

\includegraphics[height=0.4in]{illustrations/demo_parity/q9-11_POOL.png}
\begin{enumerate}
\setcounter{enumi}{8}
    \item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/demo_parity/q9_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/demo_parity/q9_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{Yes}

\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/demo_parity/q10_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/demo_parity/q10_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}
    
\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/demo_parity/q11_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/demo_parity/q11_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}

\item In your own words, explain the hiring rule. [short answer] [The rule is not shown above this question]

\item To what extent do you agree with the following statement: I am confident I know how to apply the hiring rule described above?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please select the choice that best describes your experience: When I answered the previous questions...
\begin{enumerate}
    \item I applied the provided hiring rule only.
    \item I used a combination of the provided hiring rule and my own ideas of what the correct hiring rule should be.
    \item I used only my own ideas of what the correct hiring decision should be rather than the provided hiring rule.
\end{enumerate}

\item To what extent do you agree with the following statement: I like the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item To what extent do you agree with the following statement: I agree with the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please explain your opinion on the hiring rule. [short answer]

\item Was there anything about this survey that was hard to understand or answer? [short answer]

\end{enumerate}

\paragraph{Equal Opportunity - FNR.}

Recruit-a-matic uses the following rule to determine whether Sales-a-lot’s hiring decisions were fair:
 
\emph{The fraction of qualified male candidates who do not receive job offers should equal the fraction of qualified female candidates who do not receive job offers.}

Example 1: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot received the following qualified applicants (10 female and 12 male).

\includegraphics[height=1in]{illustrations/fnr/example_1_POOL.png}

If Sales-a-lot did not send job offers to the following number of qualified applicants (5 female and 6 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/fnr/example_1b_no_offer.png}

Example 2: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot reviewed a total of 100 qualified applicants as follows (40 female and 60 male).

\includegraphics[height=2in]{illustrations/fnr/example_2_POOL.png}

If Sales-a-lot did not send job offers to the following number of qualified applicants (10 female and 15 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/fnr/example_2b_no_offer.png}

Note that in the above examples the remaining qualified applicants received job offers, but are not displayed here.

In the next section, we will ask you some questions about the information you have just read. Please note that this is not a test of your abilities. We want to measure the quality of the description you read, not your ability to take tests or answer questions.

\textbf{Please note that we ask you to apply and use ONLY the above hiring rule when answering the following questions. You will have an opportunity to state your opinions and feelings on the rule later in the survey.}

\begin{enumerate}
\setcounter{enumi}{2}
    \item Suppose a different company considered applicants for a different job. There were 200 qualified female applicants and 100 qualified male applicants,

\includegraphics[height=1.2in]{illustrations/fnr/q3_POOL.png}

and they did not send job offers to 90 qualified male applicants.

\includegraphics[height=1.3in]{illustrations/fnr/q3_male_no_offer.png}

Assuming that Recruit-a-matic reviews their decisions using the hiring rule above, how many qualified female applicants should not have received job offers?
\begin{enumerate}
    \item 190
    \includegraphics[height=1.3in]{illustrations/fnr/q3_a_no_offer.png}
    \item \correct{180}
    \includegraphics[height=1.3in]{illustrations/fnr/q3_b_no_offer.png}
    \item 160
    \includegraphics[height=1.3in]{illustrations/fnr/q3_c_no_offer.png}
    \item 150
    \includegraphics[height=1.3in]{illustrations/fnr/q3_d_no_offer.png}
\end{enumerate}

\item Assuming Recruit-a-matic reviews decisions using the hiring rule above, in which of these cases could Sales-a-lot have rejected more qualified female applicants than qualified male applicants?

\begin{enumerate}
    \item \correct{When there are more qualified female applicants than qualified male applicants (i.e., more women had low net sales at the end of the year).}
    \item When there are more female applicants than male applicants.
    \item When female applicants receive worse interview scores than male applicants.
    \item This cannot happen under the hiring rule.
\end{enumerate}

\item Consider one male applicant and one female applicant, both of whom are similarly qualified for the job (they achieve about the same net sales at the end of their first year). Is the following statement \correct{TRUE} OR FALSE: The hiring rule above allows Sales-a-lot to make a job offer to one of these applicants and not the other.

\item Consider a situation where all female applicants were unqualified (they all achieve low net sales at the end of their first year), but some of them received job offers. Is the following statement TRUE OR \correct{FALSE}: The hiring rule above requires that some job offers made to male applicants must have been made to unqualified male applicants.

\item Suppose Sales-a-lot received 100 male and 100 female applicants, and eventually made 10 job offers. Is the following statement TRUE OR \correct{FALSE}: The hiring rule above requires that even if all male applicants were unqualified (they all achieve low net sales at the end of their first year), some of the unqualified males must have received job offers.

\item Is the following statement \correct{TRUE} OR FALSE: The hiring rule above always allows Sales-a-lot to send job offers only to the most qualified applicants (those who achieve high net sales at the end of their first year).

\end{enumerate}

Consider a different scenario than the two examples above, with 6 qualified applicants -- 4 female and 2 male, as illustrated below. The next three questions each give a different potential outcome for all 6 qualified applicants (i.e., which of the 6 applicants do not receive job offers). Please indicate which of the outcomes follow the hiring rule above.

\includegraphics[height=0.4in]{illustrations/fnr/q9-11_POOL.png}
\begin{enumerate}
\setcounter{enumi}{8}
    \item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fnr/q9_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/fnr/q9_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{Yes}

\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fnr/q10_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/fnr/q10_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}
    
\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fnr/q11_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/fnr/q11_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}

\item In your own words, explain the hiring rule. [short answer] [The rule is not shown above this question]

\item To what extent do you agree with the following statement: I am confident I know how to apply the hiring rule described above?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please select the choice that best describes your experience: When I answered the previous questions...
\begin{enumerate}
    \item I applied the provided hiring rule only.
    \item I used a combination of the provided hiring rule and my own ideas of what the correct hiring rule should be.
    \item I used only my own ideas of what the correct hiring decision should be rather than the provided hiring rule.
\end{enumerate}

\item To what extent do you agree with the following statement: I like the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item To what extent do you agree with the following statement: I agree with the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please explain your opinion on the hiring rule. [short answer]

\item Was there anything about this survey that was hard to understand or answer? [short answer]
\end{enumerate}

\paragraph{Equal Opportunity - FPR.}
Recruit-a-matic uses the following rule to determine whether Sales-a-lot’s hiring decisions were fair:
 
\emph{The fraction of unqualified male candidates who receive job offers should equal the fraction of unqualified female candidates who receive job offers.}

Example 1: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot received the following unqualified applicants (10 female and 12 male).

\includegraphics[height=1in]{illustrations/fpr/example_1_POOL.png}

If Sales-a-lot sent job offers to the following number of unqualified applicants (5 female and 6 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/fpr/example_1b_offer.png}

Example 2: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot reviewed a total of 100 unqualified applicants as follows (40 female and 60 male).

\includegraphics[height=2in]{illustrations/fpr/example_2_POOL.png}

If Sales-a-lot sent job offers to the following number of unqualified applicants (10 female and 15 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/fpr/example_2b_offer.png}

Note that in the above examples the remaining unqualified applicants did not receive job offers, but are not displayed here.

In the next section, we will ask you some questions about the information you have just read. Please note that this is not a test of your abilities. We want to measure the quality of the description you read, not your ability to take tests or answer questions.

\textbf{Please note that we ask you to apply and use ONLY the above hiring rule when answering the following questions. You will have an opportunity to state your opinions and feelings on the rule later in the survey.}

\begin{enumerate}
\setcounter{enumi}{2}
    \item Suppose a different company considered applicants for a different job. There were 200 unqualified female applicants and 100 unqualified male applicants,

\includegraphics[height=1.3in]{illustrations/fpr/q3_POOL.png}

and they did send job offers to 10 unqualified male applicants.

\includegraphics[height=1.3in]{illustrations/fpr/q3_male_offer.png}

Assuming that Recruit-a-matic reviews their decisions using the hiring rule above, how many unqualified female applicants should have received job offers?
\begin{enumerate}
    \item 10
    \includegraphics[height=1.3in]{illustrations/fpr/q3_a_offer.png}
    \item \correct{20}
    \includegraphics[height=1.3in]{illustrations/fpr/q3_b_offer.png}
    \item 40
    \includegraphics[height=1.3in]{illustrations/fpr/q3_c_offer.png}
    \item 50
    \includegraphics[height=1.3in]{illustrations/fpr/q3_d_offer.png}
\end{enumerate}

\item Assuming Recruit-a-matic reviews decisions using the hiring rule above, in which of these cases could Sales-a-lot have accepted more unqualified female applicants than unqualified male applicants?

\begin{enumerate}
    \item \correct{When there are more unqualified female applicants than unqualified male applicants (i.e., more women had low net sales at the end of the year).}
    \item When there are more female applicants than male applicants.
    \item When female applicants receive worse interview scores than male applicants.
    \item This cannot happen under the hiring rule.
\end{enumerate}

\item Consider one male applicant and one female applicant, both of whom are similarly qualified for the job (they achieve about the same net sales at the end of their first year). Is the following statement \correct{TRUE} OR FALSE: The hiring rule above allows Sales-a-lot to make a job offer to one of these applicants and not the other.

\item Consider a situation where all female applicants were unqualified (they all achieve low net sales at the end of their first year), but some of them received job offers. Is the following statement \correct{TRUE} OR FALSE: The hiring rule above requires that some job offers made to male applicants must have been made to unqualified male applicants.

\item Suppose Sales-a-lot received 100 male and 100 female applicants, and eventually made 10 job offers. Is the following statement TRUE OR \correct{FALSE}: The hiring rule above requires that even if all male applicants were unqualified (they all achieve low net sales at the end of their first year), some of the unqualified males must have received job offers.

\item Is the following statement \correct{TRUE} OR FALSE: The hiring rule above always allows Sales-a-lot to send job offers only to the most qualified applicants (those who achieve high net sales at the end of their first year).

\end{enumerate}

Consider a different scenario than the two examples above, with 6 unqualified applicants -- 4 female and 2 male, as illustrated below. The next three questions each give a different potential outcome for all 6 applicants (i.e., which of the 6 applicants receive job offers). Please indicate which of the outcomes follow the hiring rule above.

\includegraphics[height=0.4in]{illustrations/fpr/q9-11_POOL.png}
\begin{enumerate}
\setcounter{enumi}{8}
    \item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fpr/q9_offer.png}
    
    Do these decisions obey the hiring rule? \correct{Yes}

\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fpr/q10_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}
    
\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/fpr/q11_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}

\item In your own words, explain the hiring rule. [short answer] [The rule is not shown above this question]

\item To what extent do you agree with the following statement: I am confident I know how to apply the hiring rule described above?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please select the choice that best describes your experience: When I answered the previous questions...
\begin{enumerate}
    \item I applied the provided hiring rule only.
    \item I used a combination of the provided hiring rule and my own ideas of what the correct hiring rule should be.
    \item I used only my own ideas of what the correct hiring decision should be rather than the provided hiring rule.
\end{enumerate}

\item To what extent do you agree with the following statement: I like the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item To what extent do you agree with the following statement: I agree with the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please explain your opinion on the hiring rule. [short answer]

\item Was there anything about this survey that was hard to understand or answer? [short answer]

\end{enumerate}

\paragraph{Equalized Odds.}
Recruit-a-matic uses the following rule to determine whether Sales-a-lot’s hiring decisions were fair:
 
\emph{The fraction of qualified male candidates who do not receive job offers should equal the fraction of qualified female candidates who do not receive job offers. Similarly, the fraction of unqualified male candidates who receive job offers should equal the fraction of unqualified female candidates who receive job offers.}

Example 1: Suppose that over the past year, Recruit-a-matic finds that Sales-a-lot received the following qualified applicants (10 female and 12 male) and unqualified applicants (10 female and 12 male).

\includegraphics[height=1in]{illustrations/eo/example_1_POOL.png}

If Sales-a-lot did send offers to the following number of unqualified applicants (left, 5 female and 6 male), and did not send job offers to the following number of qualified applicants (right, 5 female and 6 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/eo/example_1b_offer.png}
\space\space\space
\includegraphics[height=1in]{illustrations/eo/example_1b_no_offer.png}

Example 2: Suppose that over the past year, Recruit-a-lot finds that Sales-a-lot reviewed a total of 100 qualified applicants (40 female and 60 male) and 100 unqualified applicants (40 female and 60 male).

\includegraphics[height=2in]{illustrations/eo/example_2_POOL.png}

If Sales-a-lot did send offers to the following number of unqualified applicants (left, 10 female and 15 male), and did not send job offers to the following number of qualified applicants (right, 10 female and 15 male), then this would be fair according to the hiring rule (note that there are other possible outcomes that are fair according to the hiring rule).

\includegraphics[height=1in]{illustrations/eo/example_2b_offer.png}
\space\space\space
\includegraphics[height=1in]{illustrations/eo/example_2b_no_offer.png}

Note that in the above examples the remaining unqualified applicants did not receive job offers, but are not displayed here. Similarly, the remaining qualified applicants received job offers, but are not displayed here.

In the next section, we will ask you some questions about the information you have just read. Please note that this is not a test of your abilities. We want to measure the quality of the description you read, not your ability to take tests or answer questions.

\textbf{Please note that we ask you to apply and use ONLY the above hiring rule when answering the following questions. You will have an opportunity to state your opinions and feelings on the rule later in the survey.}

\begin{enumerate}
\setcounter{enumi}{2}
    \item Suppose a different company considered applicants for a different job. There were 200 qualified female applicants and 100 qualified male applicants,

\includegraphics[height=1.2in]{illustrations/eo/q3_POOL.png}

and they did not send job offers to 90 qualified male applicants.

\includegraphics[height=1.3in]{illustrations/eo/q3_male_no_offer.png}

Assuming that Recruit-a-matic reviews their decisions using the hiring rule above, how many qualified female applicants should not have received job offers?
\begin{enumerate}
    \item 190
    \includegraphics[height=1.3in]{illustrations/eo/q3_a_no_offer.png}
    \item \correct{180}
    \includegraphics[height=1.3in]{illustrations/eo/q3_b_no_offer.png}
    \item 160
    \includegraphics[height=1.3in]{illustrations/eo/q3_c_no_offer.png}
    \item 150
    \includegraphics[height=1.3in]{illustrations/eo/q3_d_no_offer.png}
\end{enumerate}

\item Assuming Recruit-a-matic reviews decisions using the hiring rule above, in which of these cases could Sales-a-lot have accepted more unqualified female applicants than unqualified male applicants?

\begin{enumerate}
    \item \correct{When there are more unqualified female applicants than unqualified male applicants (i.e., more women had low net sales at the end of the year).}
    \item When there are more female applicants than male applicants.
    \item When female applicants receive worse interview scores than male applicants.
    \item This cannot happen under the hiring rule.
\end{enumerate}

\item Consider one male applicant and one female applicant, both of whom are similarly qualified for the job (they achieve about the same net sales at the end of their first year). Is the following statement \correct{TRUE} OR FALSE: The hiring rule above allows Sales-a-lot to make a job offer to one of these applicants and not the other.

\item Consider a situation where all female applicants were unqualified (they all achieve low net sales at the end of their first year), but some of them received job offers. Is the following statement \correct{TRUE} OR FALSE: The hiring rule above requires that some job offers made to male applicants must have been made to unqualified male applicants.

\item Suppose Sales-a-lot received 100 male and 100 female applicants, and eventually made 10 job offers. Is the following statement TRUE OR \correct{FALSE}: The hiring rule above requires that even if all male applicants were unqualified (they all achieve low net sales at the end of their first year), some of the unqualified males must have received job offers.

\item Is the following statement \correct{TRUE} OR FALSE: The hiring rule above always allows Sales-a-lot to send job offers only to the most qualified applicants (those who achieve high net sales at the end of their first year).

\end{enumerate}

Consider a different scenario than the two examples above, with 6 qualified applicants -- 4 female and 2 male; and 6 unqualified applicants -- 4 female and 2 male. The next three questions each give a different potential outcome for the applicants (i.e., which of the applicants did or did not receive job offers). Please indicate which of the outcomes follow the hiring rule above.

\includegraphics[height=0.4in]{illustrations/eo/q9-11_POOL.png}
\begin{enumerate}
\setcounter{enumi}{8}
    \item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/eo/q9_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/eo/q9_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{Yes}

\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/eo/q10_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/eo/q10_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}
    
\item Sales-a-lot makes the following hiring decisions.

    \includegraphics[height=0.4in]{illustrations/eo/q11_offer.png}
    \space\space\space
    \includegraphics[height=0.4in]{illustrations/eo/q11_no_offer.png}
    
    Do these decisions obey the hiring rule? \correct{No}

\item In your own words, explain the hiring rule. [short answer] [The rule is not shown above this question]

\item To what extent do you agree with the following statement: I am confident I know how to apply the hiring rule described above?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please select the choice that best describes your experience: When I answered the previous questions...
\begin{enumerate}
    \item I applied the provided hiring rule only.
    \item I used a combination of the provided hiring rule and my own ideas of what the correct hiring rule should be.
    \item I used only my own ideas of what the correct hiring decision should be rather than the provided hiring rule.
\end{enumerate}

\item To what extent do you agree with the following statement: I like the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item To what extent do you agree with the following statement: I agree with the hiring rule?
\begin{itemize}
    \item Strongly agree
    \item Agree
    \item Neither agree nor disagree
    \item Disagree
    \item Strongly Disagree
\end{itemize}

\item Please explain your opinion on the hiring rule. [short answer]

\item Was there anything about this survey that was hard to understand or answer? [short answer]
\end{enumerate}
